Toward Smart Doors: A Position Paper

Conventional automatic doors cannot distinguish between people wishing to pass through the door and people passing by the door, so they often open unnecessarily. This leads to the need to adopt new systems in both commercial and non-commercial environments: smart doors. In particular, a smart door system predicts the intention of people near the door based on the social context of the surrounding environment and then makes rational decisions about whether or not to open the door. This work proposes the first position paper related to smart doors, without bells and whistles. We first point out that the problem not only concerns reliability, climate control, safety, and mode of operation. Indeed, a system to predict the intention of people near the door also involves a deeper understanding of the social context of the scene through a complex combined analysis of proxemics and scene reasoning. Furthermore, we conduct an exhaustive literature review about automatic doors, providing a novel system formulation. Also, we present an analysis of the possible future application of smart doors, a description of the ethical shortcomings, and legislative issues.

==> tex/2-list_of_works.tex <==
\section{Related Work}
\label{sec:related}

This section focuses on the research efforts that precede this work. It includes studies dedicated to the several automatic door systems proposed by researchers in previous years and the first attempts that use artificial intelligence in developing automatic door systems.

\luigi{@Federico, quella qui di seguito è (per ora) soltanto una lista di tutti i lavori presenti allo stato dell'arte. Nello specifico, per ognuno, ho riportato: citazione, breve descrizione, e link al codice (dove presente).}

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Intelligent Automatic Door}
\cite{jimoh2007intelligent}: This paper describes design and prototyping a voice-based door access control system for building security. In the proposed system, the access may be authorized simply by means of an enrolled user speaking into a microphone attached to the system.

\cite{song2009development}: This paper proposes an ultrasonic sensor based intelligent automatic door system which improves the performance of conventional door systems by adding more intelligent functions such that it offers more convenience to passersby and reduces power loss.

\cite{sumbul2011control}: In this paper a fuzzy logic have designed to the control of an automatic door. Input status (WS: Walking Speed and DD: Distance Door) and the output status (DOS: Door Opening Speed) is determined. According to these statuses, rule bases (25 rules) have obtained. And the rules bases have been processed by a fuzzy logic and have tried to control of an automatic door.

\cite{zhang2012intelligent}: An intelligent door control system based on the image technology is proposed and implemented. The system of miniaturization and real-time is realized by the hardware structure of double controller (FPGA+ARM). The image data is collected by a camera which is controlled by FPGA. And at the same time the grayscale is pretreated. Using the bus and ARM embedded system to communicate and the image door control algorithm is achieved by transplanting OpenCV. Experimental results show that the accuracy rate is up to 96%.

\cite{fosstveit2012intelligent}: They propose a solution by replacing the traditional sensor with the more sophisticated Microsoft Kinect depth mapping sensor allowing for skeletal tracking and feature extraction.

\cite{yang2013intelligent}: This paper presents an innovative access control system, based on human detection and path analysis, to reduce false automatic door system actions while increasing the added values for security applications. The proposed system can first identify a person from the scene, and track his trajectory to predict his intention for accessing the entrance, and finally activate the door accordingly.

\cite{nishida2014development}: Conventional automatic doors cannot distinguish between people wishing to pass through the door and people passing by the door, so they often open unnecessarily. This paper describes an intelligent door system that observes people near a door so that the door opens at the proper time and only for people who have the intention of passing through it.

\cite{lwin2015automatic}: The aim of this paper is to help users for improvement of the door security of sensitive locations by using face detection and recognition. This paper is comprised mainly of three subsystems: namely face detection, face recognition and automatic door access control.

\cite{wu2016design}: A new intelligent electronic door system was designed, which is mainly composed of microcontroller STC89C52, LCD12864, pyroelectric infrared sensor, speech synthesis, keyboard module, etc.

\cite{basha2016intelligent}: In this paper, we are demonstrating an intelligent door system using Internet of Things, which notifies intrusion by sending out email notification to the owner.

\cite{ma2018intelligent}: ASSA ABLOY is seeking a potential way of opening and closing automatic door to save the energy used by air infiltration. This thesis will provide ASSA ABLOY an intelligent swing door control system which aims to reduce more energy loss based on the consideration of human factors, product improvement cost.

\cite{kiru2020intelligent}: To address this problem, researchers have proposed solutions ranging from the use of fuzzy logic to rule-based approaches to make automatic doors better than the previous ones. In this study, an AI-based automatic door system is proposed, which uses a supervised machine learning approach to train classifiers using human body measurement.

\cite{skenderi2021dohmo}: An embedded computer vision system where multiple sensors, including intelligent cameras, are connected to actuators that regulate illumination and doors.

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Trajectory Forecasting}
\cite{owens2000application}: This paper presents an approach to the problem of automatically classifying events detected by video surveillance systems; specifically, of detecting unusual or suspicious movements.

\cite{morris2008survey}: This paper presents a survey of trajectory-based activity analysis for visual surveillance. It describes techniques that use trajectory data to define a general set of activities that are applicable to a wide range of scenes and environments.

\cite{lee2008traclass}: The proposed framework overcomes the limitations of the previous studies because trajectory partitioning makes discriminative parts of trajectories identifiable, and the two types of clustering collaborate to find features of both regions and sub-trajectories. Experimental results demonstrate that TraClass generates high-quality features and achieves high classification accuracy from real trajectory data.

\cite{nascimento2009trajectory}: This paper proposes an approach for recognizing human activities (more specifically, pedestrian trajectories) in video sequences, in a surveillance context.

\cite{anagnostopoulos2014intelligent}: We treat the problem of movement prediction as a classification task. We assume the existence of a (gradually populated/trained) knowledge base and try to compare the movement pattern of a certain object with stored information in order to predict its future locations.

\cite{monfort2015intent}: We address these two challenges, high dimensionality and uncertainty, by employing predictive inverse optimal control methods to estimate a probabilistic model of human motion trajectories. Our inverse optimal control formulation estimates quadratic cost functions that best rationalize observed trajectories framed as solutions to linear-quadratic regularization problems.

\cite{becker2018evaluation}: In recent years, there is a shift from modeling the tracking problem based on Bayesian formulation towards using deep neural networks. The evaluation is done on the publicly available TrajNet benchmark dataset, which builds up a repository of considerable and popular datasets for trajectory-based activity forecasting.

\cite{da2019survey}: In this paper we survey the state of the art in trajectory classification and compare existing methods using two different classifiers over several datasets with different characteristics, guiding the best scenarios for using each technique.

\cite{qi2020imitative}: We propose a novel imitative non-autoregressive modeling method to simultaneously handle the trajectory prediction task and the missing value imputation task. Specifically, our framework adopts an imitation learning paradigm, which contains a recurrent conditional variational autoencoder (RC-VAE) as a demonstrator, and a non-autoregressive transformation model (NART) as a learner. By jointly optimizing the two models, RC-VAE can predict the future trajectory and capture the temporal relationship in the sequence to supervise the NART learner. As a result, NART learns from the demonstrator and imputes the missing value in a non autoregressive strategy.

\cite{giuliari2021transformer}: We question the use of the LSTM models and propose the novel use of Transformer Networks for trajectory forecasting. This is a fundamental switch from the sequential step-by-step processing of LSTMs to the only-attention-based memory mechanisms of Transformers. Code available \href{https://github.com/FGiuliari/Trajectory-Transformer}{here}. 

\cite{kothari2021human}: In this work, we present an in-depth analysis of existing deep learning-based methods for modelling social interactions. We propose two domain-knowledge inspired data-driven methods to effectively capture these social interactions. To objectively compare the performance of these interaction-based forecasting models, we develop a large scale interaction-centric benchmark TrajNet++, a significant yet missing component in the field of human trajectory forecasting. Code available \href{https://github.com/vita-epfl/trajnetplusplusbaselines}{here}.

\cite{ivanovic2021rethinking}:  In this work, we take a step back and critically evaluate current trajectory forecasting metrics, proposing task-aware metrics as a better measure of performance in systems where prediction is being deployed. We additionally present one example of such a metric, incorporating planning-awareness within existing trajectory forecasting metrics.

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dataset}
\cite{ferrero2018movelets}: We extend the concept of time series shapelets for trajectories, and to the best of our knowledge, this work is the first to use shapelets in the trajectory domain. We evaluated the proposed approach with several categories of datasets, including hurricanes, vehicles, animals, and transportation means, and show with extensive experiments that our method largely outperformed state of the art works, indicating that Movelets is very promising for trajectory classification.

\cite{styles2019forecasting}:  Deep learning models that have revolutionized other areas in computer vision have seen limited application to trajectory forecasting, in part due to the lack of richly annotated training data. We address the lack of training data by introducing a scalable machine annotation scheme that enables our model to be trained using a large dataset without human annotation. In addition, we propose Dynamic Trajectory Predictor (DTP), a model for forecasting pedestrian trajectory up to one second into the future. Code available \href{https://github.com/olly-styles/Dynamic-Trajectory-Predictor}{here}.

\cite{fatima2013analysis}: In this paper, we develop a Framework for Smart Homes Dataset Analysis (FSHDA) to reflect their diverse dimensions in predefined format. It analyzes a list of data dimensions that covers the variations in time, activities, sensors, and inhabitants. For validation, we examine the effects of proposed data dimension on state-of-the-art activity recognition techniques. The results show that dataset dimensions highly affect the classifiers’ individual activity label assignments and their overall performances. The outcome of our study is helpful for upcoming researchers to develop a better understanding about the smart home datasets characteristics with classifier’s performance.



==> tex/2-related_v1.tex <==
\section{Related Work}
\label{sec:related}

This section focuses on the research efforts that precede this work. It includes studies dedicated to the several automatic door systems proposed by researchers in previous years and the first attempts that use artificial intelligence in developing automatic door systems.

\federico{Link solo per comodità nella bozza, rimossi nella versione finale. Ogni sezione è indicata 2 volte. La prima è la "versione pubblicabile", ovvero il discorso finale. La seconda indica tutte le sources a disposizione, utile durante la scrittura, e verrà rimossa nella versione finale del paper}

\subsection{Intelligent Automatic Door}
The automation of doors has seen numerous approaches and evolutions throughout the years, with \emph{smart doors} being the latest iteration in the innovation process. The different approaches can be grouped in general categories indicating their methodologies and performances.
\subsubsection{Automation through sensors} 
This is the most common approach, and can be summarized in the use of motion sensors to trigger the opening of a door.
This category has seen some evolution throughout the years, particularly in the use of different sensors: starting with classic InfraRed (IR) sensors \cite{garcia2018LowPowerSensor}, the methodology has progressed by pairing other sensors in order to improve performances. In \cite{song2009development} \cite{kim2017object} the use of Ultrasonic Sensors brought an improvement in the detection of movement, especially in outside scenarios where IR light from the sun would interfere with the IR sensor of the door. 
More recently, the use of Temperature Sensors \cite{iskandar2021automatic} \cite{supriana2021implementation}, which would only open the door if a subject's temperature did not exceed a certain treshold. This method provided a way to not only mitigate the spread on viruses (by not opening a door to feverish people), but also solved the problem of False~Positives~openings in cases where the motion detected came from an inanimated object (or small animal), since these cases could be prevented by not opening the door to subjects below a certain temperature treshold. In particular, False Positives (meaning unnecessary openings of the door) are the main problem in this category of approaches, which generally do not \emph{classify} the subjects generating the movements detected, meaning that a door would open even when not necessary if some movement was detected by the sensors at play.

\subsubsection{Automation through Detection}
With \emph{Detection} we refer to the task of \emph{recognizing people} in a scenario, usually in images. With this definition, we can describe this category's approach as the use of sensors (usually cameras) to \emph{Detect} people and open the door. This approach improves on the previous one by only opening the door to people (or specified subjects), thus reducing the number of False Positives.
The most common approach relies on cameras whose output is the fed to a Machine Learning (ML) Detection Model, whose job is to classify if the scene contains a person. 
A similar approach is presented in \cite{fosstveit2012intelligent} \cite{feng2017control}, where a \emph{Kinect} sensor and its APIs are used to detect people in the scene and open a door accordingly. 
Another interesting approach \cite{lwin2015automatic} uses a camera to perform \emph{Face Detection and Recognition}, further improving the methodology, adding a layer of security by only opening the door to authorized personnel (authenticated through \emph{Face Recognition}). 

While this category reduces the number of False Positives compared to the Sensors based Method, it still suffers from False Positives openings, for example when a person walks by the door, without the \emph{intention} of going through it. \emph{Intention} should thus be an important factor to consider when trying to reduce the number of False Positives.

\subsubsection{Automation through Intention}
As stated before, it is possible for a person to walk by a door without having the \emph{Intention} of walking through it. In these cases an automatic door should not open, and if it does, it should be considered a False Positive, meaning the system wrongly predicted the subject would need the door to be opened.
The use of \emph{Intention based} systems has seen a recent rise in popularity, mainly due to the increase of computing power which allows the training and use of more complex algorithms in a Real-Time scenario, like automated doors.
While studying the \emph{intentions} of people is hard, it can be made easier by making it explicit by the users. In \cite{jimoh2007intelligent} \cite{wu2016design} a \emph{Speech Recognition} model is used to recognize commands from the users, opening the doors accordingly. Another approach is to make \emph{intention} explicit by requesting the user to show a particular token \cite{yoon2020iot}, assume a pre-defined pose \cite{terashima2021proposal} or perform a pre-defined gesture \cite{chiu2021gesture}, all of which would need to be recognized by ML models.

These approaches clearly reduce the number of False Positives compared to the previous ones, however they introduce the risk of increasing the number of False Negatives, where the door would not open because of the mis-identification of the necessary commands, due to the innate complexity of these tasks.
Another problem of these approach is the necessity of explicit interactions from the users, which makes these approaches non usable in scenarios where the users may be unable to perform the necessary gestures.

To solve this last problem and make door automation a seamless operation, there needs to be a \emph{Detection of Implicit Intention}, where a systems needs to predict the intention of the users without them needing to perform out-of-the-ordinary tasks. 
This can be done by use of sensors, much like previous approaches, to obtain data like Walking Speed and Door Distance. This data can then be used together with some Fuzzy Rules to determine whether or not a user needs the door to be opened, resulting in the method presented in \cite{sumbul2011control}.
Other approaches estimate the intention of the users through \emph{Trajectory Forecasting} \cite{yang2013intelligent} \cite{skenderi2021dohmo}, predicting the trajectory of people in the scene (recorded with cameras) and using this information to infer the \emph{intention} to use (or not use) the door. These methods result in a seamless experience for the user who no longer needs to worry about stopping their workflow to issue commands to the system.


\subsection{Intelligent Automatic Door: sources}
\federico{Verrà rimossa}

\textbf{Standard sensors}

\cite{song2009development}: This paper proposes an ultrasonic sensor based intelligent automatic door system which improves the performance of conventional door systems by adding more intelligent functions such that it offers more convenience to passersby and reduces power loss.
\href{https://www.koreascience.or.kr/article/JAKO200921140045290.page}{Link}

\cite{garcia2018LowPowerSensor}: Low Power Sensor Node Applied to Domotic, uso di sensore wireless a basso consumo per domotica, inclusa apertura automatica di porte.
\href{
https://link.springer.com/chapter/10.1007/978-3-030-03763-5_6
}{Link}

\cite{kim2017object}: Object Recognition Performance Improvement of Door Ultrasonic Sensor. Simile ad altro Linkato, questo è del 2017. Utilizzano sensori ad ultrasuoni per migliorare le performance di sensori termici/infrarossi all'aperto, dove il sole causa problemi. È in coreano...
\href{
https://www.koreascience.or.kr/article/JAKO201713647761018.pdf
}{Link}

\cite{iskandar2021automatic}: Utilizzo di sensori di temperatura per aprire porte automaticamente. 2021, per covid.
\href{
http://ijcis.net/index.php/ijcis/article/view/42
}{Link}

\cite{supriana2021implementation}: Sensore di temperatura per aprire porte, 2021 per covid
\href{
http://iocscience.org/ejournal/index.php/mantik/article/view/1800
}{Link}

\cite{mahesh2022smart}: Aprire porta solo dopo che utente si è igenizzato mani. Fun. 2022, per covid
\href{
https://ieeexplore.ieee.org/abstract/document/9743026
}{Link}

\cite{icsilak2010smart}: Sensori wireless per domotica, con persone disabili in mente. 2010
\href{
https://www.emo.org.tr/ekler/1bd8ffbe15a3e9c_ek.pdf
}{Link}

\cite{adedayo2014design}: Porta con contatore di visitatori. 2014. Meh
\href{
http://eprints.lmu.edu.ng/193/1/Microcontroller%20Auto%20Door%20with%20Visitor%20counter.pdf
}{Link}


\textbf{Interazione Esplicita}

\cite{jimoh2007intelligent}: This paper describes design and prototyping a voice-based door access control system for building security. In the proposed system, the access may be authorized simply by means of an enrolled user speaking into a microphone attached to the system.
\href{https://d1wqtxts1xzle7.cloudfront.net/50322250/jcssp.2007.274-with-cover-page-v2.pdf?Expires=1654254765&Signature=WuV0TVpl8Q7d-bS4owoeaVymTOjSpsLkWAdgheA~6SM65vX67o4IwQNLFgNjI~aUFSucVYvNyST~aEf4ZO2djez25KDhW9qHh3Cs9i72SFNbk-xgbWNq864L7h1371skJyMcYafSPou1PPCN0kGrNnFDFXFCopFsES0gkDoP7t4s13~1UgUJxZVGJqGqm9Rf8mf58fDfL5xeFRXghPR9kj4y6JwCbYTIBFpVAzX8i291Qjuh51yQRBpfZnBVGLfFpO9RnPuMNBQB0V2P0G3MFVdrBl6PX4dFiD1yyQiV-Iibot6kj7p3QwU3reZgISm6XQ2ujIHcPc1LmvTW~EfO5g__&Key-Pair-Id=APKAJLOHF5GGSLRBV4ZA}{Link}

\cite{wu2016design}: A new intelligent electronic door system was designed, which is mainly composed of microcontroller STC89C52, LCD12864, pyroelectric infrared sensor, speech synthesis, keyboard module, etc.
\href{http://www.c-a-m.org.cn/EN/abstract/abstract4079.shtml}{Link}

\cite{terashima2021proposal}: Aprire porte solo tramite "passcodes", in questo caso frasi e pose predefinite, per ridurre falsi positivi e/o implementare sicurezza. 2021
\href{
https://dl.acm.org/doi/abs/10.1145/3472307.3484648
}{Link}

\cite{chiu2021gesture}: Multitask learning per classificazione di gesture delle mani per apertura di porte, utilizzando sensori termici. U-Net. 2021 per covid.
\href{
https://ieeexplore.ieee.org/abstract/document/9645718
}{Link}

\cite{yoon2020iot}: IoT con videocamere per aprire porte solo ad utenti autorizzati, tramite token visivo. 2020, devo approfondire per capire meglio.
\href{
https://www.koreascience.or.kr/article/JAKO202016151584643.page
}{Link}



\textbf{Detection "semplice"}

\cite{fosstveit2012intelligent}: They propose a solution by replacing the traditional sensor with the more sophisticated Microsoft Kinect depth mapping sensor allowing for skeletal tracking and feature extraction.
\href{https://ntnuopen.ntnu.no/ntnu-xmlui/handle/11250/252880}{Link}

\cite{lwin2015automatic}: The aim of this paper is to help users for improvement of the door security of sensitive locations by using face detection and recognition. This paper is comprised mainly of three subsystems: namely face detection, face recognition and automatic door access control.
\href{http://kresttechnology.com/krest-academic-projects/krest-major-projects/ECE/BTech%20%20Major%20ECE%20EMBEDDED%202016-17/Btech%20ECE%20Embedded%20Major%20BP%202016-17/81.Embedded%20Based%20Door%20Access%20Control.pdf
}
{Link}

\cite{feng2017control}: Kinect per aprire porta
\href{
http://ww.w.bncss.org/index.php/bncss/article/view/79
}{Link}




\textbf{Interazione implicita (intention)}

\cite{sumbul2011control}: In this paper a fuzzy logic have designed to the control of an automatic door. Input status (WS: Walking Speed and DD: Distance Door) and the output status (DOS: Door Opening Speed) is determined. According to these statuses, rule bases (25 rules) have obtained. And the rules bases have been processed by a fuzzy logic and have tried to control of an automatic door.
\href{https://ieeexplore.ieee.org/abstract/document/5946111}{Link}

\cite{yang2013intelligent}: This paper presents an innovative access control system, based on human detection and path analysis, to reduce false automatic door system actions while increasing the added values for security applications. The proposed system can first identify a person from the scene, and track his trajectory to predict his intention for accessing the entrance, and finally activate the door accordingly.
\href{https://www.mdpi.com/1424-8220/13/5/5923}{Link}

\cite{nishida2014development}: Conventional automatic doors cannot distinguish between people wishing to pass through the door and people passing by the door, so they often open unnecessarily. This paper describes an intelligent door system that observes people near a door so that the door opens at the proper time and only for people who have the intention of passing through it.
\href{https://ieeexplore.ieee.org/abstract/document/6907799}{Link}

\cite{kiru2020intelligent}: To address this problem, researchers have proposed solutions ranging from the use of fuzzy logic to rule-based approaches to make automatic doors better than the previous ones. In this study, an AI-based automatic door system is proposed, which uses a supervised machine learning approach to train classifiers using human body measurement.
\href{
https://ieeexplore.ieee.org/abstract/document/9293673
}{Link}

\cite{skenderi2021dohmo}: An embedded computer vision system where multiple sensors, including intelligent cameras, are connected to actuators that regulate illumination and doors.
\href{
https://ieeexplore.ieee.org/abstract/document/9568372/
}{Link}


\textbf{Not checked}

\cite{zhang2012intelligent}: An intelligent door control system based on the image technology is proposed and implemented. The system of miniaturization and real-time is realized by the hardware structure of double controller (FPGA+ARM). The image data is collected by a camera which is controlled by FPGA. And at the same time the grayscale is pretreated. Using the bus and ARM embedded system to communicate and the image door control algorithm is achieved by transplanting OpenCV. Experimental results show that the accuracy rate is up to 96\%.


\cite{basha2016intelligent}: In this paper, we are demonstrating an intelligent door system using Internet of Things, which notifies intrusion by sending out email notification to the owner.
\href{
https://www.researchgate.net/profile/Jilani-S-A-K/publication/304365504_An_Intelligent_Door_System_using_Raspberry_Pi_and_Amazon_Web_Services_IoT/links/5c42a31b92851c22a37fb1ef/An-Intelligent-Door-System-using-Raspberry-Pi-and-Amazon-Web-Services-IoT.pdf
}{Link}

\cite{ma2018intelligent}: ASSA ABLOY is seeking a potential way of opening and closing automatic door to save the energy used by air infiltration. This thesis will provide ASSA ABLOY an intelligent swing door control system which aims to reduce more energy loss based on the consideration of human factors, product improvement cost.
\href{

}{Link}


%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Trajectory Forecasting}
\cite{owens2000application}: This paper presents an approach to the problem of automatically classifying events detected by video surveillance systems; specifically, of detecting unusual or suspicious movements.
\href{
https://ieeexplore.ieee.org/abstract/document/856860
}{Link}

\cite{morris2008survey}: This paper presents a survey of trajectory-based activity analysis for visual surveillance. It describes techniques that use trajectory data to define a general set of activities that are applicable to a wide range of scenes and environments.
\href{
https://ieeexplore.ieee.org/abstract/document/4543858
}{Link}

\cite{lee2008traclass}: The proposed framework overcomes the limitations of the previous studies because trajectory partitioning makes discriminative parts of trajectories identifiable, and the two types of clustering collaborate to find features of both regions and sub-trajectories. Experimental results demonstrate that TraClass generates high-quality features and achieves high classification accuracy from real trajectory data.
\href{
https://dl.acm.org/doi/abs/10.14778/1453856.1453972
}{Link}

\cite{nascimento2009trajectory}: This paper proposes an approach for recognizing human activities (more specifically, pedestrian trajectories) in video sequences, in a surveillance context.
\href{
https://ieeexplore.ieee.org/abstract/document/5371914
}{Link}

\cite{anagnostopoulos2014intelligent}: We treat the problem of movement prediction as a classification task. We assume the existence of a (gradually populated/trained) knowledge base and try to compare the movement pattern of a certain object with stored information in order to predict its future locations.
\href{
https://ieeexplore.ieee.org/abstract/document/6807808
}{Link}

\cite{monfort2015intent}: We address these two challenges, high dimensionality and uncertainty, by employing predictive inverse optimal control methods to estimate a probabilistic model of human motion trajectories. Our inverse optimal control formulation estimates quadratic cost functions that best rationalize observed trajectories framed as solutions to linear-quadratic regularization problems.
\href{
https://www.aaai.org/ocs/index.php/AAAI/AAAI15/paper/view/9897/9671
}{Link}

\cite{becker2018evaluation}: In recent years, there is a shift from modeling the tracking problem based on Bayesian formulation towards using deep neural networks. The evaluation is done on the publicly available TrajNet benchmark dataset, which builds up a repository of considerable and popular datasets for trajectory-based activity forecasting.
\href{
https://arxiv.org/abs/1805.07663
}{Link}

\cite{da2019survey}: In this paper we survey the state of the art in trajectory classification and compare existing methods using two different classifiers over several datasets with different characteristics, guiding the best scenarios for using each technique.
\href{
https://ieeexplore.ieee.org/abstract/document/8923877
}{Link}

\cite{qi2020imitative}: We propose a novel imitative non-autoregressive modeling method to simultaneously handle the trajectory prediction task and the missing value imputation task. Specifically, our framework adopts an imitation learning paradigm, which contains a recurrent conditional variational autoencoder (RC-VAE) as a demonstrator, and a non-autoregressive transformation model (NART) as a learner. By jointly optimizing the two models, RC-VAE can predict the future trajectory and capture the temporal relationship in the sequence to supervise the NART learner. As a result, NART learns from the demonstrator and imputes the missing value in a non autoregressive strategy.
\href{
https://openaccess.thecvf.com/content_CVPR_2020/html/Qi_Imitative_Non-Autoregressive_Modeling_for_Trajectory_Forecasting_and_Imputation_CVPR_2020_paper.html
}{Link}

\cite{giuliari2021transformer}: We question the use of the LSTM models and propose the novel use of Transformer Networks for trajectory forecasting. This is a fundamental switch from the sequential step-by-step processing of LSTMs to the only-attention-based memory mechanisms of Transformers. Code available \href{https://github.com/FGiuliari/Trajectory-Transformer}{here}. 
\href{
https://ieeexplore.ieee.org/abstract/document/9412190
}{Link}

\cite{kothari2021human}: In this work, we present an in-depth analysis of existing deep learning-based methods for modelling social interactions. We propose two domain-knowledge inspired data-driven methods to effectively capture these social interactions. To objectively compare the performance of these interaction-based forecasting models, we develop a large scale interaction-centric benchmark TrajNet++, a significant yet missing component in the field of human trajectory forecasting. Code available \href{https://github.com/vita-epfl/trajnetplusplusbaselines}{here}.
\href{
https://ieeexplore.ieee.org/abstract/document/9408398
}{Link}

\cite{ivanovic2021rethinking}:  In this work, we take a step back and critically evaluate current trajectory forecasting metrics, proposing task-aware metrics as a better measure of performance in systems where prediction is being deployed. We additionally present one example of such a metric, incorporating planning-awareness within existing trajectory forecasting metrics.
\href{
https://arxiv.org/abs/2107.10297
}{Link}

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dataset}
\cite{ferrero2018movelets}: We extend the concept of time series shapelets for trajectories, and to the best of our knowledge, this work is the first to use shapelets in the trajectory domain. We evaluated the proposed approach with several categories of datasets, including hurricanes, vehicles, animals, and transportation means, and show with extensive experiments that our method largely outperformed state of the art works, indicating that Movelets is very promising for trajectory classification.
\href{
https://dl.acm.org/doi/abs/10.1145/3167132.3167225
}{Link}

\cite{styles2019forecasting}:  Deep learning models that have revolutionized other areas in computer vision have seen limited application to trajectory forecasting, in part due to the lack of richly annotated training data. We address the lack of training data by introducing a scalable machine annotation scheme that enables our model to be trained using a large dataset without human annotation. In addition, we propose Dynamic Trajectory Predictor (DTP), a model for forecasting pedestrian trajectory up to one second into the future. Code available \href{https://github.com/olly-styles/Dynamic-Trajectory-Predictor}{here}.
\href{
https://ieeexplore.ieee.org/abstract/document/8814207
}{Link}

\cite{fatima2013analysis}: In this paper, we develop a Framework for Smart Homes Dataset Analysis (FSHDA) to reflect their diverse dimensions in predefined format. It analyzes a list of data dimensions that covers the variations in time, activities, sensors, and inhabitants. For validation, we examine the effects of proposed data dimension on state-of-the-art activity recognition techniques. The results show that dataset dimensions highly affect the classifiers’ individual activity label assignments and their overall performances. The outcome of our study is helpful for upcoming researchers to develop a better understanding about the smart home datasets characteristics with classifier’s performance.
\href{
https://link.springer.com/article/10.1007/s11227-013-0978-8
}{Link}
